Very Simple Classifier: a Concept Binary Classifier toInvestigate Features Based on Subsampling and Localility

We propose Very Simple Classifier (VSC) a novel method designed to incorporate the concepts of subsampling and locality in the definition of features to be used as the input of a perceptron. The rationale is that locality theoretically guarantees a bound on the generalization error. Each feature in VSC is a max-margin classifier built on randomly-selected pairs of samples. The locality in VSC is achieved by multiplying the value of the feature by a confidence measure that can be characterized in terms of the Chebichev inequality. The output of the layer is then fed in a output layer of neurons. The weights of the output layer are then determined by a regularized pseudoinverse. Extensive comparison of VSC against 9 competitors in the task of binary classification is carried out. Results on 22 benchmark datasets with fixed parameters show that VSC is competitive with the Multi Layer Perceptron (MLP) and outperforms the other competitors. An exploration of the parameter space shows VSC can outperform MLP.

==> tables/rankings.tex <==
\begin{table*}[tbh]
	\begin{center}
	\scalebox{.8}{
	\begin{tabular}{lccccccccccccccccccccccc}
		&Avg&\rot{appendicitis}&\rot{banana}&\rot{bands}&\rot{bupa}&\rot{coil2000}&\rot{haberman}&\rot{heart}&\rot{hepatitis}&\rot{ionosphere}&\rot{magic}&\rot{mammographic}&\rot{monk-2}&\rot{phoneme}&\rot{pima}&\rot{ring}&\rot{sonar}&\rot{spambase}&\rot{spectfheart}&\rot{titanic}&\rot{twonorm}&\rot{wdbc}&\rot{wisconsin}\\
		\midrule
		VSC&3.77&5&2&3&2&2&7&1&3&1&5&5&6&6&2&2&8&5&3&5&4&4&2\\
		MLP&3.95&8&4&7&1&7&1&5&6&4&2&4&3&5&3&3&3&1&6&7&3&1&3\\
		SVC rbf&4.36&2&1&1&3&5&3&9&2&9&1&3&5&4&6&6&2&8&1&2&6&10&7\\
		AdaBoost&4.73&3&8&6&6&3&5&7&1&3&6&1&1&8&7&4&1&2&5&6&7&5&9\\
		SVC linear&4.68&1&9&2&4&1&4&4&7&5&9&2&10&9&1&9&4&4&2&8&2&2&4\\
		Random Forest&5.59&7&6&8&5&8&9&8&5&2&3&8&4&1&8&5&6&3&4&4&8&6&5\\
		K Neighbors&6.09&4&5&5&9&6&8&2&4&10&4&9&8&2&9&10&5&6&9&10&5&3&1\\
		ELM&6.82&10&3&4&7&4&6&6&9&8&7&6&7&7&5&8&9&10&7&1&9&9&8\\
		Naive Bayes&7.32&6&10&10&10&10&2&3&10&6&10&7&9&10&4&1&10&9&10&9&1&8&6\\
		Decision Tree&7.59&9&7&9&8&9&10&10&8&7&8&10&1&3&10&7&7&7&8&2&10&7&10\\
		\bottomrule
	\end{tabular}
	}
	\end{center}
	\caption{The table shows the rank for each classifier on the datasets.}
	\label{tab:rankings}
\end{table*}


==> tables/rankings2.tex <==
\begin{table*}[b]
	\begin{center}
	\scalebox{.8}{
	\begin{tabular}{lccccccccccccccccccccccc}
		&Avg&\rot{appendicitis}&\rot{banana}&\rot{bands}&\rot{bupa}&\rot{coil2000}&\rot{haberman}&\rot{heart}&\rot{hepatitis}&\rot{ionosphere}&\rot{magic}&\rot{mammographic}&\rot{monk-2}&\rot{phoneme}&\rot{pima}&\rot{ring}&\rot{sonar}&\rot{spambase}&\rot{spectfheart}&\rot{titanic}&\rot{twonorm}&\rot{wdbc}&\rot{wisconsin}\\
		\midrule
		VSC&3.50&5&1&3&2&1&7&1&3&1&4&5&6&6&2&2&8&5&3&5&3&3&1\\
		MLP&3.91&8&4&7&1&7&1&5&6&4&2&4&3&5&3&3&3&1&6&6&3&1&3\\
		SVM RBF&4.36&2&1&1&3&5&3&9&2&9&1&3&5&4&6&6&2&8&1&2&6&10&7\\
		AdaBoost&4.59&3&8&6&6&1&5&7&1&3&6&1&1&7&7&4&1&2&5&6&7&5&9\\
		SVM Linear&4.68&1&9&2&4&1&4&4&7&5&9&2&10&9&1&9&4&4&2&8&2&2&4\\
		Random Forest&5.41&7&6&8&5&8&9&8&5&1&3&8&4&1&8&5&6&3&4&2&8&6&4\\
		K Neighbors&6.05&4&5&5&9&6&8&2&4&10&4&9&8&2&8&10&5&6&9&10&5&3&1\\
		ELM&6.68&10&3&4&7&1&6&6&9&8&7&6&7&7&5&8&9&10&7&1&9&9&8\\
		Naive Bayes&7.32&6&10&10&10&10&2&3&10&6&10&7&9&10&4&1&10&9&10&9&1&8&6\\
		Decision Tree&7.59&9&7&9&8&9&10&10&8&7&8&10&1&3&10&7&7&7&8&2&10&7&10\\
		\bottomrule
	\end{tabular}
	}
	\end{center}
	\caption{Experiment 1. The table shows the rank for each classifier on the datasets.}
	\label{tab:rankings}
\end{table*}


==> tables/results.tex <==
\begin{table*}[tbh]
	\begin{center}
	\begin{tabular}{lcccccccccc}
		&\rot{VSC}&\rot{MLP}&\rot{SVM RBF}&\rot{AdaBoost}&\rot{SVM Linear}&\rot{Random Forest}&\rot{K Neighbors}&\rot{ELM}&\rot{Naive Bayes}&\rot{Decision Tree}\\
		\midrule
		appendicitis&{0.910}&{0.878}&{0.921}&{0.920}&\textbf{0.922}&{0.892}&{0.918}&{0.808}\triDown&{0.901}&{0.867}\\
		banana&{0.914}&{0.906}&\textbf{0.914}&{0.760}\triDown&{0.711}\triDown&{0.895}\triDown&{0.901}\triDown&{0.913}&{0.710}\triDown&{0.885}\triDown\\
		bands&{0.711}&{0.655}&\textbf{0.772}&{0.660}&{0.732}&{0.643}\triDown&{0.672}&{0.698}&{0.080}\triDown&{0.547}\triDown\\
		bupa&{0.772}&\textbf{0.785}&{0.759}&{0.739}&{0.756}&{0.750}&{0.662}\triDown&{0.720}&{0.511}\triDown&{0.705}\triDown\\
		coil2000&{0.969}&{0.960}\triDown&{0.968}\triDown&{0.969}&\textbf{0.969}&{0.958}\triDown&{0.966}\triDown&{0.969}\triDown&{0.101}\triDown&{0.937}\triDown\\
		haberman&{0.819}&\textbf{0.843}\triUp&{0.840}\triUp&{0.826}&{0.838}&{0.799}&{0.817}&{0.823}&{0.841}\triUp&{0.727}\triDown\\
		heart&\textbf{0.867}&{0.852}&{0.803}\triDown&{0.824}\triDown&{0.857}&{0.817}\triDown&{0.862}&{0.827}\triDown&{0.858}&{0.768}\triDown\\
		hepatitis&{0.903}&{0.869}&{0.910}&\textbf{0.926}&{0.867}\triDown&{0.893}&{0.895}&{0.803}&{0.637}\triDown&{0.842}\triDown\\
		ionosphere&\textbf{0.938}&{0.921}&{0.893}&{0.928}&{0.913}&{0.938}&{0.885}\triDown&{0.898}&{0.910}&{0.903}\\
		magic&{0.884}&{0.903}\triUp&\textbf{0.905}\triUp&{0.880}&{0.848}\triDown&{0.899}\triUp&{0.884}&{0.866}\triDown&{0.813}\triDown&{0.860}\triDown\\
		mammographic&{0.821}&{0.828}&{0.829}&\textbf{0.835}&{0.830}&{0.799}&{0.797}\triDown&{0.814}&{0.813}&{0.778}\triDown\\
		monk-2&{0.903}&{0.993}\triUp&{0.961}\triUp&\textbf{1.000}\triUp&{0.811}\triDown&{0.981}\triUp&{0.886}&{0.887}&{0.868}&\textbf{1.000}\triUp\\
		phoneme&{0.892}&{0.895}&{0.904}\triUp&{0.871}\triDown&{0.843}\triDown&\textbf{0.929}\triUp&{0.917}\triUp&{0.871}\triDown&{0.821}\triDown&{0.911}\triUp\\
		pima&{0.834}&{0.822}&{0.813}\triDown&{0.812}\triDown&\textbf{0.835}&{0.804}\triDown&{0.804}\triDown&{0.814}\triDown&{0.816}\triDown&{0.764}\triDown\\
		ring&{0.969}&{0.960}\triDown&{0.889}\triDown&{0.955}\triDown&{0.785}\triDown&{0.929}\triDown&{0.767}\triDown&{0.851}\triDown&\textbf{0.980}\triUp&{0.882}\triDown\\
		sonar&{0.630}&{0.685}&{0.696}&\textbf{0.716}&{0.669}&{0.647}&{0.666}&{0.593}&{0.564}&{0.634}\\
		spambase&{0.930}&\textbf{0.951}\triUp&{0.857}\triDown&{0.948}\triUp&{0.939}\triUp&{0.945}\triUp&{0.919}\triDown&{0.806}\triDown&{0.829}\triDown&{0.914}\triDown\\
		spectfheart&{0.874}&{0.863}&\textbf{0.885}&{0.865}&{0.881}&{0.869}&{0.828}\triDown&{0.856}\triDown&{0.744}\triDown&{0.848}\triDown\\
		titanic&{0.860}&{0.848}\triDown&{0.862}&{0.848}\triDown&{0.847}\triDown&{0.862}&{0.832}\triDown&\textbf{0.865}\triUp&{0.842}\triDown&{0.862}\\
		twonorm&{0.977}&{0.977}&{0.967}\triDown&{0.962}\triDown&{0.978}&{0.939}\triDown&{0.970}\triDown&{0.938}\triDown&\textbf{0.979}&{0.843}\triDown\\
		wdbc&{0.975}&\textbf{0.978}&{0.875}\triDown&{0.972}&{0.976}&{0.968}&{0.975}&{0.908}\triDown&{0.944}\triDown&{0.949}\triDown\\
		wisconsin&{0.976}&{0.974}&{0.970}&{0.964}\triDown&{0.973}&{0.973}&\textbf{0.976}&{0.968}&{0.971}&{0.958}\triDown\\
		\midrule
		Average&0.879&0.879&0.872&0.872&0.854&0.870&0.855&0.841&0.752&0.836\\
		Median&0.898&0.886&0.887&0.875&0.847&0.894&0.885&0.854&0.825&0.861\\
		\bottomrule
	\end{tabular}
	\end{center}
	\caption{The table reports the experimental F1 measure we obtained on the analyzed datasets. The best results for each dataset are marked in bold. Results that are statistically better and worse with respect to our method are marked with \triDown ~  and with \triUp ~ respectively.}
	\label{tab:results}
\end{table*}


==> tables/results2.tex <==
\begin{table*}[t]
	\begin{center}
	\begin{tabular}{lcccccccccc}
		&\rot{VSC}&\rot{MLP}&\rot{SVM RBF}&\rot{AdaBoost}&\rot{SVM Linear}&\rot{Random Forest}&\rot{K Neighbors}&\rot{ELM}&\rot{Naive Bayes}&\rot{Decision Tree}\\
		\midrule
		appendicitis&{0.910}&{0.878}&{0.921}&{0.920}&\textbf{0.922}&{0.892}&{0.918}&{0.808}\triDown&{0.901}&{0.867}\\
		banana&\textbf{0.914}&{0.906}&\textbf{0.914}&{0.760}\triDown&{0.711}\triDown&{0.895}\triDown&{0.901}\triDown&{0.913}&{0.710}\triDown&{0.885}\triDown\\
		bands&{0.711}&{0.655}&\textbf{0.772}&{0.660}&{0.732}&{0.643}\triDown&{0.672}&{0.698}&{0.080}\triDown&{0.547}\triDown\\
		bupa&{0.772}&\textbf{0.785}&{0.759}&{0.739}&{0.756}&{0.750}&{0.662}\triDown&{0.720}&{0.511}\triDown&{0.705}\triDown\\
		coil2000&\textbf{0.969}&{0.960}\triDown&{0.968}\triDown&\textbf{0.969}&\textbf{0.969}&{0.958}\triDown&{0.966}\triDown&\textbf{0.969}\triDown&{0.101}\triDown&{0.937}\triDown\\
		haberman&{0.819}&\textbf{0.843}\triUp&{0.840}\triUp&{0.826}&{0.838}&{0.799}&{0.817}&{0.823}&{0.841}\triUp&{0.727}\triDown\\
		heart&\textbf{0.867}&{0.852}&{0.803}\triDown&{0.824}\triDown&{0.857}&{0.817}\triDown&{0.862}&{0.827}\triDown&{0.858}&{0.768}\triDown\\
		hepatitis&{0.903}&{0.869}&{0.910}&\textbf{0.926}&{0.867}\triDown&{0.893}&{0.895}&{0.803}&{0.637}\triDown&{0.842}\triDown\\
		ionosphere&\textbf{0.938}&{0.921}&{0.893}&{0.928}&{0.913}&\textbf{0.938}&{0.885}\triDown&{0.898}&{0.910}&{0.903}\\
		magic&{0.884}&{0.903}\triUp&\textbf{0.905}\triUp&{0.880}&{0.848}\triDown&{0.899}\triUp&{0.884}&{0.866}\triDown&{0.813}\triDown&{0.860}\triDown\\
		mammographic&{0.821}&{0.828}&{0.829}&\textbf{0.835}&{0.830}&{0.799}&{0.797}\triDown&{0.814}&{0.813}&{0.778}\triDown\\
		monk-2&{0.903}&{0.993}\triUp&{0.961}\triUp&\textbf{1.000}\triUp&{0.811}\triDown&{0.981}\triUp&{0.886}&{0.887}&{0.868}&\textbf{1.000}\triUp\\
		phoneme&{0.892}&{0.895}&{0.904}\triUp&{0.871}\triDown&{0.843}\triDown&\textbf{0.929}\triUp&{0.917}\triUp&{0.871}\triDown&{0.821}\triDown&{0.911}\triUp\\
		pima&{0.834}&{0.822}&{0.813}\triDown&{0.812}\triDown&\textbf{0.835}&{0.804}\triDown&{0.804}\triDown&{0.814}\triDown&{0.816}\triDown&{0.764}\triDown\\
		ring&{0.969}&{0.960}\triDown&{0.889}\triDown&{0.955}\triDown&{0.785}\triDown&{0.929}\triDown&{0.767}\triDown&{0.851}\triDown&\textbf{0.980}\triUp&{0.882}\triDown\\
		sonar&{0.630}&{0.685}&{0.696}&\textbf{0.716}&{0.669}&{0.647}&{0.666}&{0.593}&{0.564}&{0.634}\\
		spambase&{0.930}&\textbf{0.951}\triUp&{0.857}\triDown&{0.948}\triUp&{0.939}\triUp&{0.945}\triUp&{0.919}\triDown&{0.806}\triDown&{0.829}\triDown&{0.914}\triDown\\
		spectfheart&{0.874}&{0.863}&\textbf{0.885}&{0.865}&{0.881}&{0.869}&{0.828}\triDown&{0.856}\triDown&{0.744}\triDown&{0.848}\triDown\\
		titanic&{0.860}&{0.848}\triDown&{0.862}&{0.848}\triDown&{0.847}\triDown&{0.862}&{0.832}\triDown&\textbf{0.865}\triUp&{0.842}\triDown&{0.862}\\
		twonorm&{0.977}&{0.977}&{0.967}\triDown&{0.962}\triDown&{0.978}&{0.939}\triDown&{0.970}\triDown&{0.938}\triDown&\textbf{0.979}&{0.843}\triDown\\
		wdbc&{0.975}&\textbf{0.978}&{0.875}\triDown&{0.972}&{0.976}&{0.968}&{0.975}&{0.908}\triDown&{0.944}\triDown&{0.949}\triDown\\
		wisconsin&\textbf{0.976}&{0.974}&{0.970}&{0.964}\triDown&{0.973}&{0.973}&\textbf{0.976}&{0.968}&{0.971}&{0.958}\triDown\\
		\midrule
		Average&0.879&0.879&0.872&0.872&0.854&0.870&0.855&0.841&0.752&0.836\\
		Median&0.898&0.886&0.887&0.875&0.847&0.894&0.885&0.854&0.825&0.861\\
		\bottomrule
	\end{tabular}
	\end{center}
	\caption{Experiment 1. The table reports the experimental F1 measure we obtained on the analyzed datasets. The best results for each dataset are marked in bold. Results that are statistically better and worse with respect to our method are marked with \triDown ~  and with \triUp ~ respectively.}
	\label{tab:results}
\end{table*}

